Low Emission Building Control with Zero-Shot Reinforcement Learning

Heating and cooling systems in buildings account for 31% of global energy use, much of which are regulated by Rule Based Controllers (RBCs) that neither maximise energy efficiency nor minimise emissions by interacting optimally with the grid. Control via Reinforcement Learning (RL) has been shown to significantly improve building energy efficiency, but existing solutions require access to building-specific simulators or data that cannot be expected for every building in the world. In response, we show it is possible to obtain emission-reducing policies without such knowledge a priori--a paradigm we call zero-shot building control. We combine ideas from system identification and model-based RL to create PEARL (Probabilistic Emission-Abating Reinforcement Learning) and show that a short period of active exploration is all that is required to build a performant model. In experiments across three varied building energy simulations, we show PEARL outperforms an existing RBC once, and popular RL baselines in all cases, reducing building emissions by as much as 31% whilst maintaining thermal comfort. Our source code is available online via https://enjeeneer.io/projects/pearl/

==> tables/decomp.tex <==
\begin{table}[!t] 
\centering
\caption{\label{table: agent decomposition}\textbf{Agent Decomposition.} Mean daily reward for four instantiations of PEARL varying the choice of network and planning algorithm. The \textit{Oracle} is reported as a baseline. Experiments conducted in the Mixed-Use environment for one year.}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{lll}
\toprule
                             & Deterministic   & Probabilistic  \\
\midrule
Random Shooting (RS) & $-7.11e5$ & $-7.30e5$   \\
MPPI & $\mathbf{-5.28e5}$  & $-5.65e5$   \\

\midrule
Oracle & $-4.77e5$
\end{tabular}
}
\end{table}


==> tables/results.tex <==
\begin{table*}[!ht] 
\centering
\caption{\label{table:results}\textbf{\textit{Energym} Performance.} Results for all agents across our three \textit{Energym} environments. We define the temperature infraction metric as the percentage of days where mean building temperature falls outside the target range [19, 24], and latency as the mean compute time each agent requires to select an action given its policy measured in seconds per action. Results are averaged across 3 runs and presented as mean $\pm$ standard deviation, except for the Oracle which has converged on a policy prior to deployment with multiple runs showing the same performance.}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{llllll}
\toprule
                             & Agent   & Emissions (tCO$_2$) & Temp. Infractions &  Latency & Mean Reward \\
\midrule
\multirow{5}{*}{\rotatebox[]{90}{Mixed-Use}}   & RBC     &  $68.09 \scriptstyle{\pm0.00}$ & $2.47\% \scriptstyle{\pm0\%}$   & -- & --                   \\
                             & PPO     &   $48.80 \scriptstyle{\pm10.35}$  & $48.49\%\scriptstyle{\pm6.08\%}$ & $\textbf{0.021} \scriptstyle{\pm0.01}$  & $-1.47e7 \scriptstyle{\pm2.84e6}$ \\
                             & SAC & $48.80 \scriptstyle{\pm0.14}$ & $\mathbf{0\%}\scriptstyle{\pm0\%}$ &  $0.028 \scriptstyle{\pm0.02}$  & $-6.02e5 \scriptstyle{\pm3.85e4}$ \\
                             & MPC-DNN &    $48.03 \scriptstyle{\pm0.46}$ & $13.42\%\scriptstyle{\pm0.59\%}$ &  $0.030 \scriptstyle{\pm0.01}$ & $-1.12e6 \scriptstyle{\pm3.47e4}$ \\
                             & \textbf{PEARL} & $\mathbf{46.67 \scriptstyle{\pm0.09}}$ & $0.55\%\scriptstyle{\pm0.08\%}$ & $0.870 \scriptstyle{\pm 0.15}$ & $\mathbf{-5.76e10^5} \scriptstyle{\pm 2.12e10^3} $\\
                             \hline
                             & Oracle & $45.49$  & $0\%$ & $0.027$  &  $-4.77e5$ \\
\hline
\multirow{5}{*}{\rotatebox[]{90}{Office}}   & RBC     &    $\mathbf{9.61} \scriptstyle{\pm0.00}$ & $1.64\% \scriptstyle{\pm0\%}$& --     & --             \\
                             & PPO     & $12.14 \scriptstyle{\pm0.31}$ & $31.51\%\scriptstyle{\pm7.19\%}$ & $\mathbf{0.018} \scriptstyle{\pm0.006}$ & $-2.26e6 \scriptstyle{\pm 1.07e6}$ \\
                             & SAC & $11.87 \scriptstyle{\pm0.01}$ & $6.58\% \scriptstyle{\pm1.12\%}$  & $0.025 \scriptstyle{\pm0.01}$ & $-2.75e5 \scriptstyle{\pm 2.03e4}$ \\
                             & MPC-DNN & $11.93 \scriptstyle{\pm0.022}$ & $9.86\%\scriptstyle{\pm0.84\%}$ & $0.029 \scriptstyle{\pm0.001}$ & $-5.50e5 \scriptstyle{\pm2.89e4}$ \\
                             & \textbf{PEARL}   &  $10.45 \scriptstyle{\pm0.07}$ &  $\mathbf{1.52\%} \scriptstyle{\pm0\%}$ & $0.845 \scriptstyle{\pm 0.14}$ & $\mathbf{-5.51e10^4} \scriptstyle{\pm1.82e10^3}$ \\
                             \hline
                             & Oracle & $8.08$  & $2.47\%$ & $0.023$   &  $-2.63e4$ \\
\hline
\multirow{5}{*}{\rotatebox[]{90}{Sem. Centre}} & RBC     & $\mathbf{19.74} \scriptstyle{\pm0.00}$ &  $\mathbf{0\%} \scriptstyle{\pm0\%}$&  --   & --             \\
                             & PPO     &   $20.01 \scriptstyle{\pm0.27}$ &  $51.23\%\scriptstyle{\pm14.99\%}$  &  $\mathbf{0.028} \scriptstyle{\pm 0.01}$ & $-4.15e6 \scriptstyle{\pm9.67e5}$ \\
                             & SAC & $20.37 \scriptstyle{\pm0.08}$ & $29.32\%\scriptstyle{\pm1.87\%}$  & $0.033 \scriptstyle{\pm0.02}$  & $-1.95e6 \scriptstyle{\pm7.11e4}$ \\
                             & MPC-DNN &  $20.44 \scriptstyle{\pm0.02}$    & $49.13\%\scriptstyle{\pm0.56\%}$  & $0.035 \scriptstyle{\pm0.001}$  & $-2.45e6 \scriptstyle{\pm3.26e4}$ \\
                             & \textbf{PEARL}   &    $20.02 \scriptstyle{\pm0.10}$ & $\mathbf{0\%}\scriptstyle{\pm0\%}$  & $0.911 \scriptstyle{\pm 0.17}$  & $\mathbf{-1.18e10^6} \scriptstyle{\pm1.50e10^3}$ \\
                             \hline
                             & Oracle & $19.75$  & $0\%$ & $0.031$  &  $-1.14e6$ \\
\hline 
\end{tabular}}
\end{table*}
